Effectiveness of Adversarial Examples and Defenses for Malware Classification

Artificial neural networks have been successfully used for many different classification tasks including malware detection and distinguishing between malicious and non-malicious programs. Although artificial neural networks perform very well on these tasks, they are also vulnerable to adversarial examples. An adversarial example is a sample that has minor modifications made to it so that the neural network misclassifies it. Many techniques have been proposed, both for crafting adversarial examples and for hardening neural networks against them. Most previous work has been done in the image domain. Some of the attacks have been adopted to work in the malware domain which typically deals with binary feature vectors. In order to better understand the space of adversarial examples in malware classification, we study different approaches of crafting adversarial examples and defense techniques in the malware domain and compare their effectiveness on multiple datasets.

==> tabels/attacks_overview.tex <==
\begin{table*}[t]
	\centering
\begin{tabular}{ | m{5cm} | m{3cm}| m{3cm} | m{3cm} | }
	\hline
	Paper & Attack & Effectiveness & Dataset \\
	\hline \hline
	Generating Adversarial Malware Examples for Black-Box Attacks Based on {GAN} & GAN gets used to transform Malware into adversarial samples & TPR from 95\% lowered to >1\% & 180k malware examples; collected from malwr.com \\
	\hline
%	Malware Detection in Adversarial Settings: Exploiting Feature Evolutions and Confusions in Android Apps & Feature Evolutions and Confusions & 60\% & Drebin \\
%	\hline
%	Black-Box Attacks against {RNN} based Malware Detection Algorithms & Geherative RNN & Accuracy decrease from 90\% to >12\% (based on victim model) & 180 examples from malwr.com \\
%	\hline
	Adversarial Examples for Malware Detection & JSMA & 63\% & Drebin \\
	\hline
	Attack and Defense of Dynamic Analysis-Based, Adversarial Neural Malware Classification Models & Feature Enabling/Disabling & 2.5\% - 27\% successfull AE & Windows PE files \\
	\hline
	Adversarial Deep Learning for Robust Detection of Binary Encoded Malware & rFGSM \& dFGSM & 99.7\% evasion rate & Windows PE files \\
	& BGA & 99.7\% evasion rate & Windows PE files \\
	\hline
	& BCA & 41.7\% evasion rate & Windows PE files \\
	\hline
%	Generic Black-Box End-to-End Attack Against State of the Art API Call Based Malware Classifier & Insert API in random postion of call squence & Effectiveness 89\%-100\% & Windows PE dataset\\
%	\hline
\end{tabular}
\end{table*}

==> tables/defense_overview.tex <==
\begin{table*}
	\centering
	\begin{tabular}{ | m{5cm} | m{3cm}| m{3cm} | m{3cm} | }
	  \hline
	  Paper & Defense & Effectiveness & Dataset \\
	  \hline \hline
	
	  SecureDroid: Enhancing Security of Machine Learning-based Detection Against Adversarial Android Malware Attacks & Feature Selection and Ensemble & 70\% vs 5\% undefended & Properatirey Dataset from Comodo \\
	  \hline
	  Adversary Resistant Deep Neural Networks with an Application to Malware Detection & Ranom feautre nullification & 63\% resitance & Windows audit logs  \\
	  \hline
	  Adversarial Examples for Malware Detection & Distillation & No improvement & Drebin \\
	  \hline
	  & Adversarial Training &  Misclassification drops from 63\% to 40\%& Drebin \\
	  \hline
	  Attack and Defense of Dynamic Analysis-Based, Adversarial Neural Malware Classification Models & Distillation & 27\% success rate degressed to 14\% & Windows PE files \\
	  \hline
	  & Ensemble & 27\% success rate degressed to 6\% & Windows PE files \\
	  \hline
	  Adversarial Deep Learning for Robust Detection of Binary Encoded Malware & Adversarial training with saddle point formulation & successfull AE creation from 99.7\% down to ~10\%  & Windows PE files \\
	  \hline
	\end{tabular}
\end{table*}

==> tables/defenses/adv_training.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrr}
		\toprule
		Attack  						& undefended	& defended	\\
		\midrule
		natural                     	& 11.7			& 2.7		\\
		dfgsm\_k                    	& 100.0			& 7.8 \\
		rfgsm\_k                    	& 100.0			& 7.8 \\
		bga\_k                      	& 11.7			& 3.9 \\
		bca\_k                   		& 13.7			& 3.9	\\
		JSMA                        	& 100.0			& 27.5 \\
		random\_inc\_neg            	& 11.7			& 3.9 \\
		dec\_pos                    	& 100.0			& 100.0	\\
		inc\_neg                    	& 100.0			& 27.5 \\
		random\_dec\_pos            	& 100.0			& 100.0\\
		random\_dec\_pos\_inc\_neg  	& 96.1			& 25.5 \\
		dec\_pos\_inc\_neg          	& 100.0			& 25.5 \\
		malgan                      	& 77.1			& 	\\
		\bottomrule
	\end{tabular}
	\caption{Comparison of the defended an undefended network. The defended network was trained with \aexs created with $dFGSM_k$ }
	\label{def_train_table}
\end{table}

==> tables/defenses/distillation.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrr}
		\toprule
		Attack  						& undefended	& defended	\\
		\midrule
		natural                     	& 11.7			&  12.0	\\
		dfgsm\_k                    	& 100.0			& 100.0 \\
		rfgsm\_k                    	& 100.0			& 100.0 \\
		bga\_k                      	& 11.7			& 100.0	\\
		bca\_k                   		& 13.7			& 31.4	\\
		JSMA                        	& 100.0			& 100.0 \\
		random\_inc\_neg            	& 11.7			& 13.7	\\
		dec\_pos                    	& 100.0			& 100.0	\\
		inc\_neg                    	& 100.0			& 100.0	\\
		random\_dec\_pos            	& 100.0			& 100.0 \\
		random\_dec\_pos\_inc\_neg  	& 96.1			& 90.2 	\\
		dec\_pos\_inc\_neg          	& 100.0			& 100.0	\\
		malgan                      	& 77.1			& 	\\
		\bottomrule
	\end{tabular}
	\caption{Evasion rates in \% of various attacks on the undefended and defended with Distillation at temperature 10. Models are trained on \apds }
	\label{def_dist_table}
\end{table}

==> tables/defenses/ensemble.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrrrrr}
		\toprule
		Attack &						undefended 	& Ensemble	\\
		\midrule
		natural                     	& 11.7		& 8.7		\\
		dfgsm\_k                    	& 100.0		& 100.0		\\
		rfgsm\_k                    	& 100.0		& 100.0		\\
		bga\_k                      	& 11.7		& 100.0		\\
		bca\_k                   		& 13.7		& 17.6		\\
		JSMA                        	& 100.0		& 100.0		\\
		random\_inc\_neg            	& 11.7		& 15.7		\\
		dec\_pos                    	& 100.0		& 100.0		\\
		inc\_neg                    	& 100.0		& 100.0		\\
		random\_dec\_pos            	& 100.0		& 100.0		\\
		random\_dec\_pos\_inc\_neg  	& 96.1		& 98.0		\\
		dec\_pos\_inc\_neg          	& 100.0		& 100.0		\\
		malgan                      	& 77.1		&\\
		\bottomrule
	\end{tabular}
	\caption{Comparison of the different attacks applied to an ensemble of networks}
	\label{def_ensemlbe}
\end{table}





==> tables/defenses/nullification.tex <==
\begin{table}
	\centering
	\begin{tabular}{lrr}
		\toprule
		Attack  						& undefended	& defended	\\
		\midrule
		natural                     	& 11.7			& 85.6\\
		dfgsm\_k                    	& 100.0			& 13.7 \\
		rfgsm\_k                    	& 100.0			&  9.8 \\
		bga\_k                      	& 11.7			& 72.5\\
		bca\_k                   		& 13.7			& 68.6	\\
		JSMA                        	& 100.0			& 100.0 \\
		random\_inc\_neg            	& 11.7			& 3.9 \\
		dec\_pos                    	& 100.0			& 96.1	\\
		inc\_neg                    	& 100.0			& 100.0 \\
		random\_dec\_pos            	& 100.0			&  86.3\\
		random\_dec\_pos\_inc\_neg  	& 96.1			& 51.0\\
		dec\_pos\_inc\_neg          	& 100.0			& 100.0\\
		malgan                      	& 77.1			& 	\\
		\bottomrule
	\end{tabular}
	\caption{Evasion rates in \% of various attacks on the undefended and defended with Random feature nullification at a rate of 0.4. The model was trained on \apds }
	\label{def_null_table}
\end{table}

==> tables/feature_selection.tex <==
\begin{table}
	\centering
	\begin{tabular}{|c| c c|} 
		\hline
		\# features & acc. malware & acc. benign \\ 
		\hline
		500 & 0.892 & 0.996 \\ 
		1000 & 0.892 & 0.996 \\
		5000 & 0.92 & 0.997 \\
		\hline
	\end{tabular}
	\caption{Accuracy of the classifier when on the test set}
	\label{feature_selection_table}
\end{table}
